"Newspaper Eat" Means "Not Tasty": A Taxonomy and Benchmark for Coded Language in Real-World Chinese Online Reviews

Coded language is an important part of human communication. It refers to cases where users intentionally encode meaning so that the surface text differs from the intended meaning and must be decoded to be understood. Current language models handle coded language poorly. Progress has been limited by the lack of real-world datasets and clear taxonomies. This paper introduces CodedLang, a dataset of 7,744 Chinese Google Maps reviews, including 900 reviews with span-level annotations of coded language. We developed a seven-class taxonomy that captures common encoding strategies, including phonetic, orthographic, and cross-lingual substitutions. We benchmarked language models on coded language detection, classification, and review rating prediction. Results show that even strong models can fail to identify or understand coded language. Because many coded expressions rely on pronunciation-based strategies, we further conducted a phonetic analysis of coded and decoded forms. Our code and dataset are publicly available. Together, our results highlight coded language as an important and underexplored challenge for real-world NLP systems.

==> latex/sections/2-related_work.tex <==
\paragraph{Natural Language Processing Methods for Coded Languages.}
%\looseness=-1
Prior NLP work showed that coded language is hard to analyze due to its dependence on context, cultural knowledge, polysemy, and limited labeled data~\cite{ji2018creative}.
Decoding could be further complicated in multilingual settings, where translation systems and multilingual language models misinterpret coded expressions due to misleading cross-language word similarity~\cite{kallini2025false}.
Open challenges included balancing opacity and interpretability, modeling personalized and multilingual coding strategies, and handling the rapid evolution of code phrases. 
While these challenges were known, prior work lacked task formulations and datasets grounded in real-world review platforms. 
Our work addressed this gap by formulating coded reviews as an NLP task and introducing \dataset, a curated dataset of real-world coded reviews.

Existing studies focused on encoding and decoding mechanisms.
\citet{ji2018creative} showed how users encoded meaning to bypass censorship while remaining intelligible to in-group audiences, supporting functions such as discussing sensitive topics and expressing negative opinions indirectly. 
%Extending this work to online reviews, 
\citet{kim2021trkic} found that Korean speakers on Google Maps used morphological, phonological, optical, and semantic strategies to make reviews intelligible only to in-group readers.
\citet{cho2021google} also categorized intentionally noisy text by interpretation boundaries.
However, these studies did not capture how users systematically hide negative sentiment inside positive or neutral reviews, nor did they provide span-level annotations for this behavior.
Coded language has also been studied in political discourse as dog whistles, which are expressions that appear innocuous to general audiences but convey specific meanings to targeted in-groups~\cite{mendelsohn2023dogwhistles, xu2021blow}.
%Prior work showed that dog whistles evade toxicity detection and require world knowledge to interpret~\cite{mendelsohn2023dogwhistles, xu2021blow}. 
%[\changye{this part might get heated up - just be careful on word choice, or simply not mention it at all}]
This line of work focused on ideological signaling rather than everyday consumer communication and did not consider how coded language interacted with ratings or machine translation.
%\kenneth{Is this true? Don't they?} 


\paragraph{Phonetic and Orthographic Substitution.}
Early NLP work treated phonetic and orthographic variation as noise to be normalized~\cite{saito2014morphological}.
More recent studies have shown that such variations were deliberately used as coding strategies.
In Chinese internet language, homophonic substitutions and character-level perturbations encode meaning implicitly and require phonological reasoning and shared background knowledge for interpretation~\cite{xu2021blow, ma2025reasoning}.
Benchmarks showed that large language models (LLMs) struggle with these substitutions and often rely on memorized patterns rather than systematic reasoning~\cite{ma2025reasoning, ma2025phonothink}.
Related work in content moderation also showed that homophones, emoji substitutions, and visually similar characters degraded toxic language detection performance~\cite{xiao2024toxicloakcn}.
Recent work also explored countermeasures, showing that simple LLM-based approaches could partially counter algospeak~\cite{fillies2024simple}.
However, this line of work treats surface manipulation as an attack rather than a communication strategy. 
Our work instead studies how real users use phonetic and orthographic substitutions to express negative evaluations while avoiding detection.


%However, this line of work largely treated surface-form manipulation as an adversarial artifact rather than a communicative strategy.
%Our work reframed phonetic and orthographic substitution as part of a broader set of intentional coding practices used by real users to express negative evaluations while avoiding detection, and grounded our analysis in a dataset drawn from natural user behavior.
%grounded this analysis in a dataset derived from naturalistic review behavior.



%These studies exposed model weaknesses but abstracted away from user intent and communicative goals.
%While prior work exposed model vulnerabilities to surface-form manipulation, recent studies showed that simple LLM-based methods could partially counter algospeak, albeit without explicit modeling of user intent or communicative context~\cite{fillies2024simple}.
%\kenneth{I'm not entirely sure this is true? Did they ignore user intention?}
%Our work connected these surface-form strategies to user motivations by analyzing how they were used to embed negative sentiment in real-world Chinese reviews.

%------------- dead kitten ------------
\begin{comment}
  

%Prior work on encoding and decoding has long examined how meaning is constructed and interpreted under constraints. In communication theory, encoding refers to how senders shape messages using shared or assumed codes, while decoding captures how receivers interpret those messages within specific social and cultural contexts. Hall’s encoding/decoding model emphasizes that meaning is not transmitted directly but produced through interpretive processes shaped by asymmetries between production and reception contexts \cite{hall1980encoding}. Such asymmetries often lead to divergent interpretations, a phenomenon that closely parallels ambiguity and subjectivity in NLP tasks such as disambiguation and text classification.
%Hall further argues that even seemingly “natural” codes are culturally constructed, highlighting that meaning is contingent rather than inherent. This insight motivates computational perspectives that treat language understanding as an interpretive process grounded in context, background knowledge, and social convention rather than surface form alone.
\changye{any specific rationale not using $\textbackslash$subsection here?}

\changye{how these related works demonstrate the gap you aim to bridge in this paper? Technically we don't need to repeat/rephrase the methods of the related words - we can summarize with the \textbf{main} takeaways and how do their work motivates ours. For example, work1, work2, work3 investigate coded language and phonetic/orthographic substitution in language x, y and z. However, they do not xxxx. Our study seek to bridge this gap by introducing xxxx}

\paragraph{NLP for Coded Languages.}
%\textbf{Coded Language in Online Communication} 
%Prior natural language processing (NLP) [\changye{if NLP is used here jsut once, you can delete (NLP)}] 
NLP work has examined how encoding and decoding operate in creative coded language. \citet{ji2018creative} analyzes how users deliberately encode meaning to bypass censorship while remaining intelligible to in-group audiences. They illustrate coded language used for a variety of purposes: discussing sensitive information while avoiding censorship, masking illegal activity such as drug dealing, plain slang in a particular domain, such as cutesy language, and expressing strong emotion or making fun. Decoding coded language is challenging due to reliance on synonymy, polysemy, contextual ambiguity, cultural knowledge, shifting meanings over time, and the lack of labeled data. 
\citet{ji2018creative} identified several open problems, including the need and difficulty of balancing opacity and interpretability, the challenges of personalized coding strategies and multilingualism, and the time-sensitivity of code phrases as they evolve with decoding machines and human decoders over time. 

Similar to Chinese coded reviews, \citet{kim2021trkic} also found that, in Google Maps place reviews, Korean speakers also deliberately craft text that is intelligible only to in-group Korean readers to reduce interpersonal burden, and convey authentic evaluations within their community. They identify four strategies used to trick translation systems: morphological (e.g., code-switching), morpho-phonological (e.g., glottalization), optical (e.g., character substitution), and semantic (e.g., sarcasm). Additionally, \citet{cho2021google} categorizes intentionally noisy user-generated text by interpretation boundaries, distinguishing whether content is accessible to peers while remaining opaque for others.

Other than online reviews, coded expressions are commonly represented as dog-whistles in the political domain. \citet{mendelsohn2023dogwhistles} study dogwhistles that convey distinct meanings to general and in-group audiences, and show that such rhetoric evades both toxicity detection and reliable interpretation by large language models. Also, \citet{xu2021blow} collected a Chinese \textsc{DogWhistle} dataset for cant understanding through gamification crowdsourcing, demonstrating that interpreting coded expressions requires common sense and world knowledge beyond lexical cues. 


\paragraph{Phonetic and Orthographic Substitution.}
Prior work has studied how intentionally non-canonical text that remains interpretable to humans challenges automated systems. Early work on noisy text normalization focuses on handling spelling variants, phonetic substitutions, and informal lexical forms in social media, primarily treating them as surface-level noise to be corrected for downstream processing \cite{saito2014morphological}.

More recent studies emphasize the deliberate and strategic nature of such substitutions in online communication. In Chinese Internet language, homophonic substitutions and character-level perturbations are widely used to encode meaning implicitly, requiring phonological reasoning, contextual inference, and shared background knowledge for interpretation \cite{xu2021blow, ma2025reasoning}. These phenomena have been formalized as reasoning benchmarks, showing that large language models struggle to restore or interpret phonetic substitutions reliably and often rely on memorized mappings rather than systematic phonological reasoning \cite{ma2025reasoning, ma2025phonothink}.

Related work has also examined phonetic and orthographic substitutions in content moderation. Cloaking perturbations such as homophones, emoji substitutions, and visually similar characters significantly degrade offensive language detection performance, highlighting the vulnerability of NLP systems to intentional surface-form manipulation \cite{xiao2024toxicloakcn, fillies2024simple}.

%\cite{ma2025reasoning} Reasoning or memorization? investigating LLMs’ capability in restoring Chinese Internet homophones

%\cite{xiao2024toxicloakcn} ToxiCloakCN: Evaluating Robustness of Offensive Language Detection in Chinese with Cloaking Perturbations

%\cite{ma2025phonothink} PhonoThink: Improving Large Language Models’ Reasoning on Chinese Phonological Ambiguities

%\cite{saito2014morphological} Morphological analysis for Japanese noisy text based on character-level and word-level normalization

%\cite{li2024llms} When llms meet cunning texts: A fallacy understanding benchmark for large language models

%\cite{fillies2024simple} Simple llm based approach to counter algospeak


%may be cite in phonetic analysis \cite{kallini2025false} False Friends Are Not Foes: Investigating Vocabulary Overlap in Multilingual Language Models 

  
\end{comment}

==> latex/sections/3-data.tex <==
\input{latex/tables/taxonomy}

We curated \dataset, a dataset of 7,744 online reviews, of which 900 contain coded language. 
Each coded-language review includes span-level annotation(s) indicating the coding strategy, as defined by our taxonomy.
This section overviews the construction and analysis of \dataset.


%\dataset contained \textbf{900 reviews containing coded language} out of 7,744 manually annotated reviews.

%These 7,744 items include the 5,391 annotated restaurant reviews from the Pilot Study, as well as cases surfaced throughout the iterations.
%\paragraph{What are Coded Languages?}
%When curating \dataset, 
We defined \textbf{coded language} as \textit{the intentional encoding or obfuscation of meaning, in which the surface form differs from the intended meaning and decoding is required for interpretation}.
Importantly, not all socially opaque 
%[\changye{is this a commonly used phrase? how about \textit{non-dominant}? \textit{under-represented} is another candidate but it is a blocked word for NIH...}] 
language qualifies as coded language. 
Dialect, jargon, and multilingual text can be socially opaque because they rely on shared community knowledge, but they are not considered coded language unless the meaning is intentionally disguised through an explicit encoding mechanism, such as phonetic, orthographic, or symbolic substitutions. 
In contrast, coded language is socially opaque because it is encoded: understanding it requires actively decoding the surface form to recover the intended meaning.


%Importantly, not all socially opaque language applies coded language. 
%Dialect, jargon, and multilingual text can be socially opaque because they rely on shared community knowledge. 
%While dialectal expressions, jargon, or multilingual text may introduce interpretation boundaries for out-group readers, they are not considered coded language unless meaning is intentionally disguised through an explicit encoding mechanism, such as phonetic, orthographic, or symbolic substitutions. 
%In contrast, coded language is socially opaque because it is encoded: understanding requires decoding the surface form to recover the intended meaning. 



\subsection{Data Sources and Pre-Processing\label{sec:data-source}}
% Xiaohongshu + media
% Phenomenon in Google reviews
% 23 golden examples
% Large-scale Google review corpus

\paragraph{Initial Coded-Language Examples.}
We first observed news articles reporting Chinese-speaking users employing coded language to express dissatisfaction in Google Reviews for overseas businesses~\cite{shine2024newspaper, radii2024coded, yahoo_news_2025}. 
These cases were originally shared on social media platforms such as Xiaohongshu (Rednote) and Threads, where users discussed the opacity and in-group interpretability of such reviews and shared additional examples they had encountered.\footnote{For example, a Xiaohongshu post titled ``This is the first time I've seen real Chinese encryption hahaha'', and a Threads post said ``Saw a review that only Taiwanese people can understand, thank you, kind soul!'', both highlighted community awareness of such coded expressions.}
%\kenneth{A footnote for a sentence should occur after the sentence's period.}
Therefore, we collected 23 reviews containing coded language that were shared on social media or reported in news articles. 
These reviews serve as an initial seed set, providing concrete examples of real-world coded expressions and guiding our large-scale mining of low-frequency coded reviews. 

\paragraph{Real-World Google Maps Reviews.}
Building on this seed set, we further screened for coded-language instances in massive Google Maps reviews. 
We used two Google Maps review datasets:
{\em (i)} 1.77 million restaurant reviews~\cite{li2022uctopic} and 
{\em (ii)} 666 million local reviews~\cite{yan2023personalized}.
%\kenneth{What's the diff (qualitatively) between these two? As we mention (i) only gave us few example but (ii) gave us a lot more, we need to set up that by mentioning how they're different a bit.}
%The dataset is multilingual, including English, Spanish, Chinese, and other languages.
These reviews were multilingual and covered U.S. businesses, including restaurants and hotels.
Each review included a user ID, a business ID, the original review text, ratings, and an English translation of the review when the original was not in English.
%\kenneth{I revised the order of some texts above, trying to make it more clear. See if they're accurate.}
%Based
%collected by~\citeauthor{li2022uctopic} and~\citeauthor{yan2023personalized}, including 1.77 million restaurant reviews and 666 million local reviews in the United States.
%The local reviews include various businesses such as restaurants, hotels, and hospitals. 
%The Google Maps Review datasets include the user ID, business ID, original review text, ratings, and an English translation of the review if the original review is not in English.
We then selected reviews containing at least one Chinese character,
%using a regular–expression–based Unicode filter. This process 
which yielded 5,391 Chinese-language reviews from the restaurant review dataset and 112,521 from the local review dataset. 
This set included reviews written in Simplified and Traditional Chinese, with some mixed with English and other languages.\footnote{Here, \emph{Traditional Chinese} refers to written Chinese in traditional characters, including varieties such as Taiwan Mandarin and Cantonese.}
Section~\ref{sec:data-mining} described our process of finding reviews that contain coded languages from this set.
%as described in Section~\ref{sec:data-mining}.

%We used this corpus of Chinese Google Maps reviews in the United States as the target dataset for large-scale coded-language mining.

\subsection{Constructing \dataset Dataset\label{sec:data-mining}}

%\subsection{Mining Coded-Language Reviews\label{sec:data-mining}}
%0. collect 23 golden data from rednote and news media. 
%1 manually annotate 5391 restaurant reviews, which lead to 20 coded examples. The coded language usage is very rare in real life. 
%2. collect an initial coded language dictionary based on golden data from rednote and news media, and the 5391 annotations. 
%3. pinyin leakage in translation then human annotate the filtered results 
%4. Update dictionary 
%5. N-gram matching with dictionary then human annotate the filtered results 
%6. Combined EMNLP 25' Weibo homophone dictionary 7. N-gram matching with dictionary then human annotate the filtered results 
%8. Synthesize 7 coded language classes, annotate the coded data with multi-label coded language classes

%Automatically identifying coded languages at scale is challenging.
We used an iterative, human-in-the-loop mining process to identify coded languages in large-scale Google Maps reviews.
%\kenneth{Use past tense when possible. I fixed a few; not sure I caught them all.}
Two of the authors served as annotators in this process.

%this iterative process yields 900 Google Maps reviews containing coded language out of 7,744 manually annotated reviews, with the remaining reviews labeled as non-coded.

%The 7,744 annotations comprise the 5,391 restaurant reviews annotated in the pilot study, and additional candidate reviews surfaced during iterative filtering.




\paragraph{Pilot Study.}
We collected 23 gold examples of coded language from social media and news media discussions (sources described in Section~\ref{sec:data-source}).
%, where users explicitly describe and interpret coded expressions used in online reviews. 
To estimate real-world prevalence, we manually annotated 5,391 U.S. restaurant reviews (created in Section~\ref{sec:data-source}). 
We identified only 19 reviews (0.35\%) that used coded language, confirming that it is a rare phenomenon in this domain.
%\kenneth{I know we talked about this, but why coded lang are more common in local reviews?}
We also found that most coded expressions occur at the \textit{phrase level} rather than the sentence level, meaning they can often be decoded using limited local context.
A dictionary-based table lookup covering common phrases, combined with substantial human validation, should capture a large portion of real-world cases.



%We also learned that most coded expressions occur at the \textit{phrase level} rather than at the \textit{sentence level}.
%Namely, coded expressions rarely rely on the sentence-level context or information to decode, so a dictionary-based approach combined with a lot of human validation effrot should be able to capture a lot of cases.

%\kenneth{What does this mean? }

%%\eg, ``\begin{CJK}{UTF8}{gbsn}炒鸡\end{CJK}'' in ``\begin{CJK}{UTF8}{gbsn}图片里的都炒鸡好吃\end{CJK}'',


\paragraph{Step 1: Seed Dictionary Construction.}
We first annotated the specific text spans that contained coded language in all examples (\eg,``\begin{CJK}{UTF8}{gbsn}虾\end{CJK}'' in ``\begin{CJK}{UTF8}{gbsn}真的是虾到爆\end{CJK}'') from Pilot Study, where \begin{CJK}{UTF8}{gbsn}虾\end{CJK} (xia1, shrimp) is a homophonic substitution for \begin{CJK}{UTF8}{gbsn}瞎\end{CJK} (xia1, absurd), and then aggregated these annotated spans to form a dictionary.
%\kenneth{TODO: Update with real examples.}
The initial dictionary contained 100 coded spans. %184 were final spans, the initial dictionary has 100 spans, but many are not effective in mining.

\paragraph{Step 2: Candidate Retrieval and Validation.}
Using this dictionary, we applied string matching across the entire review corpus to retrieve candidate reviews containing dictionary entries. 
To further expand coverage, we also included reviews whose English machine translations contained Pinyin, a phonetic system for Chinese that uses the Latin alphabet to represent pronunciation, since this indicates potential machine translation challenges. 
All candidate reviews were then manually validated. 
%by this paper's authors.


%Using the dictionary, we applied string matching over the whole review corpus to retrieve candidate reviews, which are then manually validated. 
%Using this dictionary, we applied string matching across the entire review corpus to retrieve candidate reviews that contained dictionary entries, and then manually validated these candidates.
%To further expand coverage, we also included all the reviews whose English machine translations contained Pinyin, a phonetic system for Chinese that uses the Latin alphabet to represent pronunciation, as candidates, since this indicates potential machine translation challenges.
%To further expand coverage, we also treated all the reviews where their English machine transaltion contianed Pinyin, phonetic system for Mandarin Chinese that uses the Latin alphabet to represent pronunciation, as candidate because this signify potential MT challenges.
%examined pinyin leakage in machine-translated reviews to surface additional candidate coded expressions.
%Pinyin is the phonetic system for Mandarin Chinese that uses the Latin alphabet to represent pronunciation. %\ruyuan{add 1 sentence explain how to do the pinyin leakage filtering.}\kenneth{Do not use the phrase ``pinyin leakage''; just explain what you did in plain English.}

\paragraph{Step 3: Dictionary Expansion and Iterative Bootstraping.}
The validated reviews from Step 2 went through the same span-annotation process described in Step 1, and the newly annotated spans were added to the dictionary. 
The updated dictionary was then used to retrieve additional coded-language reviews from the corpus, and this process was repeated iteratively.
We continued the bootstrapping process until convergence, defined as an iteration in which no new validated coded-language spans were identified and no additional coded-language reviews were retrieved.
%\kenneth{TODO: Add stopping condition. When/how did you stop the iteration?}
To further improve coverage, we also incorporated all word entries from an external homophone dictionary derived from Weibo and Tieba data~\cite{ma2025reasoning} during this iterative process.

As a result, \dataset contained \textbf{900 reviews containing coded language} out of 7,744 manually annotated reviews.
These 7,744 items include the 5,391 annotated restaurant reviews from the Pilot Study, as well as cases surfaced throughout the iterations.

\paragraph{Annotating Coded Language Classes.}
Based on the accumulated coded-language instances, we developed a taxonomy of seven coded-language categories (Section~\ref{sec:taxonomy}) and annotated each review using multi-label class assignments. 
%We describe the taxonomy in detail in Section~\ref{sec:taxonomy}. 
During annotation, annotators first identified whether a review contained coded language, then marked the exact text spans that were coded. 
Each coded span, consisting of one or more characters, was assigned a single category corresponding to its primary encoding strategy.  
It is possible for a single span to involve multiple encoding mechanisms. But for annotation consistency and downstream evaluation clarity, we adopted a one-to-one span–category mapping, assigning each span to its dominant encoding strategy. Our annotation decision was based on both surface form and intended meaning. While some expressions may involve layered transformations, we categorize them according to the most salient observable mechanism. For example, the expression `` 
\begin{CJK}{UTF8}{gbsn}铁\end{CJK}\includegraphics[height=1.2em]{latex/figures/hamburger.png}\includegraphics[height=1.2em]{latex/figures/hamburger.png}'' derives from the phrase ``\begin{CJK}{UTF8}{gbsn}铁憨憨\end{CJK}'' (tie3 han1 han1, meaning ``silly''). The transformation involves an intermediate phonetic substitution \begin{CJK}{UTF8}{gbsn}憨\end{CJK} (han1, silly) to \begin{CJK}{UTF8}{gbsn}汉\end{CJK} (han4), to \begin{CJK}{UTF8}{gbsn}汉堡\end{CJK} (han4 bao3, hamburger) which is  \includegraphics[height=1.2em]{latex/figures/hamburger.png}, but the final surface form primarily manifests as emoji substitution. Therefore, it is labeled under emoji substitution in our taxonomy. 
A review could contain multiple spans using different strategies and thus receive multiple coded-language labels. This annotation process resulted in 184 unique coded spans across the dataset. While each span was assigned a single encoding category, its decoded meaning could vary depending on contextual usage.



\paragraph{Inner-Annotator Agreements.}
During the iterative bootstrapping phase, the first author manually labeled all items returned by the process and included all labeled items, both coded and non-coded, in \dataset. 
The second author then independently annotated the entire \dataset. 
They achieved high agreement on whether a review contained coded language (Cohen's kappa = 0.99), which was calculated on the annotated data before resolving disagreements.. At the span level, annotators also showed strong consistency, with 98\% of identified spans overlapping between annotators. Recurring disagreements primarily arose in distinguishing dialectal variation from intentionally coded language. In some cases, regional phonetic spellings resembled coded substitutions, requiring annotators to determine whether a form reflected deliberate encoding or ordinary dialectal expression. For example, \begin{CJK}{UTF8}{gbsn}里格楞\end{CJK} was a candidate of coded expression, but was later identified as a Beijing dialect term meaning `pull strings'. We labeled it as non-coded language, as its surface form directly reflects its intended meaning, despite posing an interpretation barrier for those unfamiliar with the dialect.
All disagreements were resolved through discussion to reach consensus, which determined the final released labels.
%\kenneth{TODO: (1) I wrote this part. Is this accurate? (2) Update the kappa.}


%The two annotators achieved high agreement on whether a review contained coded language (Cohen's kappa = 0.9X) and strong agreement on the identification of coded spans within reviews (Cohen's kappa = XXX) in their initial annotations. 
%All disagreements were resolved through collaborative discussion to reach a consensus.


%\paragraph{Data Statistics.}


%Our procedure yielded \textbf{900 Google Maps reviews containing coded language} out of 7,744 manually annotated reviews, with the remaining reviews labeled as non-coded, which were all included in \dataset.
%These 7,744 annotations include the 5,391 restaurant reviews from Pilot Study, as well as cases identified throughout the iterations.


%The validated reviews from Step 2 were then added to the dictionary, and n-gram filtering is re-applied over the corpus.
%This process is repeated iteratively, including the incorporation of an external homophone dictionary derived from Weibo and Tieba data\footnote{Weibo is China's leading microblogging platform, similar to X. Tieba is a topic-based Chinese online forum, similar to Reddit.} \cite{ma2025reasoning}. Through multiple rounds of automatic filtering and human validation, we inductively refine the decision boundary of what constitutes coded language. In total, this iterative process yields 900 Google Maps reviews containing coded language out of 7,744 manually annotated reviews, with the remaining reviews labeled as non-coded. The 7,744 annotations comprise the 5,391 restaurant reviews annotated in the pilot study, and additional candidate reviews surfaced during iterative filtering.

%Two of the authors served as annotators, achieving a Cohen's kappa agreement score of [\ruyuan{To Add}] on the annotations. (or move to the taxonomy section)



\subsection{Taxonomy of Coded Language\label{sec:taxonomy}}
%Based on the accumulated coded-language instances, we synthesize a taxonomy of seven coded-language categories and annotate each review with multi-label class assignments, enabling fine-grained analysis. A single review may contain one or more coded spans, each consisting of one or multiple characters. While each coded span is assigned a single coded-language category as its primary encoding strategy, a review may contain multiple spans employing different strategies. Then that review will be labeled with multiple coded-language classes.





%Through multiple rounds of automatic filtering and human validation, we inductively refine the decision boundary of what constitutes coded language.
%Table~\ref{tab:taxonomy} summarizes the taxonomy, including concise definitions and representative examples.
%Through multiple rounds of filtering and human validation, 
We inductively refined the decision boundaries of each category through repeated discussions between the two annotators through multiple rounds of review. 
Table~\ref{tab:taxonomy} summarizes the final, converged taxonomy, including concise definitions and representative examples.
Figure~\ref{fig:category_dist} shows the distribution of coded-language categories. Homophone-based strategies are the most prevalent, followed by phonetic and orthographic substitutions, while cipher-like expressions and cross-lingual phonetic encoding are rarer.




\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{latex/figures/Code_Lang_Distribution.pdf}
    \caption{Distribution of coded language categories in the annotated dataset.}
\label{fig:category_dist}
% dialect 有一些common phrase其实也许不include比较好，巴适得板 很地区化的表达，但咋，贼 是非常common的表达不局限于北方方言了，（北方文化入侵。。/不是）说出来大家都知道，well 大家可能是指简中用户？ 这样的话会dialect删掉300+
% 12/28/8:55pm 决定还是把咋 和 贼删掉，not all dialect and colloquial expression are coded. Coded language is more reflected on interpretation difficulty and boundary (reflectede on rednote comments thematic analysis!)
%哩哏愣 defintely hard to understand unless for beijing people, 玉蜀黍 is not less iterpretatble outside taiwanese, but 咋，贼 originate from dialects are now commonly used across region. 
\end{figure}

%\subsection{Statistics of \dataset}





%\paragraph{Distribution of Coded-Language Categories.}
%Our annotated dataset contains 900 coded reviews and 6,844
%non-coded reviews, reflecting the rarity of coded language in naturally occurring Google Maps reviews. 



==> latex/sections/4-evaluation.tex <==
Using \dataset, we evaluated the capability of LLMs to handle real-world coded language across three NLP tasks: 
{\em (i)} coded language detection, 
{\em (ii)} coded language classification, and 
{\em (iii)} review rating prediction.

%[Application part]:
%Coded language existence detection task
%Review Score Prediction
\subsection{Coded Language Detection\label{sec:detection-task}}

\paragraph{Experimental Setups.}
We assessed LLMs' ability to detect coded language in reviews using a binary classification task. 
We benchmarked a diverse set of modern English and Chinese LLMs, including GPT-5-mini~\cite{openai2025gpt5mini}, Gemini-2.5-Flash~\cite{comanici2025gemini25pushingfrontier}, Qwen2.5-7B-Instruct~\cite{qwen2025qwen25technicalreport}, DeepSeek-V3.2~\cite{deepseekai2025deepseekv32pushingfrontieropen} and Llama-3.1-8B-Instruct~\cite{llama3_1}.
Models were instructed to identify whether a review contains coded language and output a binary prediction. 
Our prompt included the definition of coded language along with few-shot examples drawn from our taxonomy.
We evaluated classification performance using precision, recall, and F$_1$ score.
%Because coded-language instances are substantially rarer than non-coded reviews, we paid more attention to precision. 

\paragraph{Results.}

\input{latex/tables/detection}
From the Table \ref{tab:detection_results}, we found DeepSeek-V3.2 has a balanced tradeoff between precision and recall, and has the highest F$_1$ score in the coded language detection. Gemini-2.5-Flash has the highest recall, which captures the majority of coded expressions at the cost of reduced precision. On the other side, Qwen2.5-7B-Instruction has the highest precision.
%\changye{I think we can just simply say which one reaches the highest recall/precision, without the which means part}
Comparing across four models, there is no single model that dominates across all metrics.%, showing the tradeoff in coded language detection. 

\input{latex/tables/classification}
\subsection{Coded Language Classification\label{sec:classification-task}}

\paragraph{Experimental Setups.}
%Beyond binary detection, we further evaluate language models’ ability to classify coded language into fine-grained categories, to study whether LLMs understand how meaning is encoded. 
We formulated coded language classification as a multi-label classification task, where a review may apply multiple coded language strategies to encode its message. Our prompts provide concise definitions of each coded-language category along with a few-shot representative examples. Given a review, models are instructed to produce a structured output with three fields: (1) classes, a list of coded-language categories applied in the review; (2) evidence, a list of exact text spans copied from the review that support the classification; and (3) a brief explanation justifying the decision. The output classes and the evidence of the coded span would be empty if no coded language is detected. Models are evaluated against annotations derived from our taxonomy and measured using precision, recall, and F$_1$ score.


\paragraph{Results.}
We reported the results of the coded-language classification using DeepSeek-V3.2. Results for other models are provided in the Appendix \ref{sec:additional_classification}. Table \ref{tab:classification_by_class} reports multi-label classification performance across coded language categories. To account for class imbalance, we reported per-class performance metrics, allowing a granular assessment across categories. Cipher expressions achieved the highest F$_1$ and precision, indicating that they are easier to identify than other categories. Cross-Lingual Phonetic Encoding had the highest recall but lowest precision and F$_1$, which tells that the model can not identify this category clearly. This might be influenced by the limited sample size of the Cross-Lingual Phonetic Encoding Category. The Homophones, Phonetic, Orthographic, and Emoji Substitutions achieved F$_1$ scores ranging from 0.42 to 0.59, indicating that these phenomena remained challenging for current models.


\subsection{Review Rate Prediction\label{sec:rating-prediction-task}}
\input{latex/tables/prediction}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{latex/figures/prediction_mse_by_ratings.png}
    \caption{Rating-wise mean squared error (MSE) for review rating prediction under different textual representations. Results were predicted by \texttt{GPT-5-mini}. Sample sizes for each rating level were shown below the x-axis, reflecting imbalance across ratings.}
    \label{fig:rating_pred}
\end{figure}


\paragraph{Experimental Setups.}
We examine review rate prediction to understand how coded language affects models' ability to infer users' intended star ratings. While ratings are commonly treated as proxies for sentiment, reviews that use coded language may express evaluative intent indirectly, introducing additional ambiguity. Considering the misalignment between ratings and review content, we manually validated the pairs of ratings and reviews. We found that ratings are generally consistent with review sentiment, with only seven reviews rated four or five that express negative content. 

The review rating prediction was evaluated on Mean Squared Error (MSE). To investigate the effect of coded language, we construct multiple formats of the same review text: (1) Non-coded reviews as original; (2) Coded reviews as original; (3) Character-based masked reviews, where each coded characters is replaced with a [CODE] token; (4) Span-based masked reviews, where consecutive coded tokens are replaced with a single [CODE-SPAN]; and (5) Decoded reviews, where coded expressions are replaced with their intended meaning using a dictionary derived from annotation. 

\paragraph{Results.}
Across all models in Table ~\ref{tab:rating_pred_mse}, the MSE on coded reviews is larger than on non-coded reviews, indicating higher prediction error under coded language. It shows that coded language disrupted sentiment signals relevant for rating prediction. GPT-5-mini showed the most robust performance across review formats, with consistently low MSE, so we further examined its predictions stratified by rating groups.

Figure~\ref{fig:rating_pred} presents rating-wise prediction error across different textual representations of reviews. Prediction errors were low for extreme ratings (1 and 5), indicating that strongly expressed sentiment was relatively easy to infer even in the presence of coded or masked language. In contrast, 3-star reviews exhibited the highest error, reflecting the inherent ambiguity of mixed or neutral evaluative intent. Notably, for intermediate ratings (2-4), masked reviews have lower error than decoded and coded reviews, suggesting that coded expressions can introduce misleading surface cues and that literal decoding does not always clarify intent.

%\kenneth{I moved the following to review score prediction part. Don't need to mention this in the dataset.------ If we don't have time, we can also remove the following paragraph.}

%\paragraph{Coded Language and Review Ratings.}
As an additional analysis, we found that
coded language was significantly associated with lower ratings in Google Reviews ($p<0.001$). 
Coded language tended to appear in relatively concise reviews under extreme sentiment conditions, even though negative reviews were longer overall ($p<0.001$). 
%Detailed statistical analyses are in the 
Appendix~\ref{sec:stat} shows the detailed analysis.


%Notes: just current draft and write up, will update with comprehensive model resutls.

==> latex/sections/5-analysis.tex <==
%[Linguistics Analysis]:
%Segmentation, Tokenization, POS tag, syntax Analysis (need some exploration)


%\begin{figure*}[htbp]
%\centering
%\subfigure[Pinyin]{
%  \includegraphics[width=0.48\textwidth]{latex/figures/pinyin_cer.pdf}
%  \label{fig:pinyin}
%}
%\hfill
%\subfigure[IPA]{
%  \includegraphics[width=0.48\textwidth]{latex/figures/ipa_cer.pdf}
%  \label{fig:ipa}
%}
%\caption{The average error rate for substitutions, deletions, and insertions per class for Pinyin (a) and IPA (b), ranking descendingly by the total number of errors for each class.}
%\label{fig:cer}
%\end{figure*}

LLMs often performed poorly on coded language, but it remained unclear which factors drive this performance drop. 
In \dataset, many coded reviews relied on pronunciation-based strategies, which raised an interesting question: 
%This observation motivated a focused question: 
\textbf{Does phonetic similarity between coded expressions and their intended meanings make coded language easier for LLMs to process?}
We conducted a set of analyses to answer this question.
%Our hypothesis was that coded language that sounded closer to its intended meaning would be easier for LLMs to interpret than coded language that sounded very different.

\input{latex/tables/cer}
\input{latex/tables/mse_by_class}

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{latex/figures/CER-Pinyin_largerfont.pdf}
\caption{The average error rate for substitutions, deletions, and insertions per class using Pinyin representations, ranked by the total number of errors per class.}
\label{fig:pinyin}
\end{figure}
%\kenneth{If no space, we can keep IPA one and move Pinyin to Appendix.}

\paragraph{Measuring Pronunciation Similarity.}
We measured phonetic similarity between coded expressions and their decoded meanings. 
We used tools to annotate Pinyin~\cite{huang2025pypinyin} and International Phonetic Alphabet (IPA) representations~\cite{taubert2025pinyintoipa} for each coded-decoded span pair in \dataset, excluding the Cipher and Orthographic Substitution classes.
%\kenneth{TODO: Cite the tool used.}
Tones in Pinyin were annotated from 1 to 4 and mapped to IPA tone contours accordingly (1 to \tone{55}, 2 to \tone{35}, 3 to \tone{313}, and 4 to \tone{51}). 
We used character error rate (CER), a common evaluation metric in automatic speech recognition (ASR), to quantify the phonetic similarity between coded and decoded spans. In ASR, CER is computed as the normalized sum of 
substitutions ($S$), 
deletions ($D$), and 
insertions ($I$) over the total number of characters ($N$) between the ASR-generated utterance (hypothesis) and verbatim utterance (reference)~\citep{inproceedings} (Equation~\ref{eq:cer}).
%where a lower CER indicates a lower \textit{proportion} of incorrectly transcribed characters against the verbatim transcript, indicating a better performance.
In our analysis, a lower CER indicates greater pronunciation similarity between the coded expression and its decoded form.
We treated each phoneme in IPA and syllable in Pinyin as a character, and computed pairwise CER for each pair of decoded span (reference) and coded span (hypothesis). Some pinyin abbreviations consist only of consonant initials, which cannot be directly mapped to IPA without a vowel. In such cases, we follow the common convention used by Chinese speakers when reading pinyin initials aloud, using pronunciation for each alphabet letter without tone to ensure pronounceability before converting to IPA. This avoids generating transduction error [UNK] tokens during IPA conversion, while we acknowledge that this transformation may introduce higher IPA error rate. 
%\kenneth{TODO: Add citation here}
%\kenneth{So CER can technically larger than 1? Why Fig 4 has value over 1??}
%\changye{yes - it's a proportion of incorrectly transcribed words/tokens over the max number of tokens}
\begin{equation}
\text{CER} = \frac{S+D+I}{N}
\label{eq:cer}
\end{equation}
Figure~\ref{fig:CER_example} illustrates how CER is computed using Pinyin and IPA representations for the same coded expression and its decoded form, including substitution, deletion, and insertion errors.
\begin{figure}[h]
\centering
\includegraphics[width=1\linewidth]{latex/figures/Phonetic_Example.pdf}
\caption{
Example of CER based on Pinyin and IPA representations.
}
\label{fig:CER_example}
\end{figure}

\subsection{Findings}

\paragraph{Phonetic Error Patterns Across Categories.}

%The average Pinyin CER of annotated Pinyin for Ambiguous Homophone, Emoji Substitution, Non-Lexical Substitution, Phonetic Substitution, and Cross-Lingual Phonetic Encoding yielded 0.33, 0.29, 0.22, 0.49, and 1.23, respectively. 
%The average CER of annotated IPA yielded 0.43, 0.25, 0.29, 0.56, and 2.31, respectively, for each class. 
As shown in Table~\ref{tab:cer_pinyin_ipa}, cross-lingual phonetic encoding yielded the highest CER, highlighting the difficulty of cross-language pronunciation mapping. Non-lexical homophones showed the lowest CER, reflecting relatively high phonetic similarity despite semantic ambiguity. 
Figure~\ref{fig:pinyin} shows the average substitution, deletion, and insertion error rates across coded language categories computed using Pinyin, following Equation~\ref{eq:error_rate}. Corresponding results using IPA are reported in Appendix~\ref{app:IPA}.

\begin{equation}
    \text{Error Rate} = \frac{\text{total \# of S/I/D}}{\text{total \# of S+I+D}}
    \label{eq:error_rate}
\end{equation}


We observed that the Phonetic Substitution class reached the highest number of deletions for both Pinyin and IPA. This observation was primarily driven by the use of Pinyin initials, which reduced multi-syllabic words to only Pinyin consonants and subsequently led to failures in the IPA conversion. For example, ``\texttt{rmb}'' was abbreviated from \texttt{\textbf{r}en2 \textbf{m}in2 \textbf{b}i4} (Chinese Yuan).
%As the initials lack sufficient phonological information, the IPA conversion produces a direct English IPA for each syllable. 
We also observed a cross-lingual case where ``\texttt{ww}'' was coded for \begin{CJK}{UTF8}{gbsn}哈哈\end{CJK} (haha, laughter), similar to \texttt{lol} (lots of laughs). The origin of \texttt{w} was abbreviated from \begin{CJK}{UTF8}{min}わら\end{CJK} (\texttt{warai}, laughter) in Japanese. In addition, substitutions reached the second most frequent error type across all coded language categories. For example, \texttt{\textbf{ji}n1 ho\textbf{u4} \textbf{xia2}} (\begin{CJK}{UTF8}{gbsn}金厚呷\end{CJK}, non-lexical homophones for `really delicious' in Taiwanese) was substituted for \texttt{\textbf{zhe}n1 h\textbf{a}o\textbf{3} \textbf{chi1}} (\begin{CJK}{UTF8}{gbsn}真好吃\end{CJK}, really delicious). 
This suggested a high degree of phonetic interference, in which the target sounds were replaced by phonetically similar but intentionally incorrect variants.
%the error type distribution across the coded language categories.

\paragraph{Phonetic Similarity and Rating Prediction Error.}
%The MSE between user-generated and predicted rating in the full dataset [\changye{this refers to the full review dataset}] for ambiguous homophone, emoji, non lexical homophone, phonetic, and transliteration yielded 0.31, 0.56, 0.43, 0.52, and 0.86, respectively. 
%The average pairwise pinyin and IPA CER for these classes were 0.49, 0.58, 0.30, 0.62, and 1.36, 0.57, 0.83, 0.37, 0.87, and 2.60, respectively.
%\kenneth{Can we add a few words here to respond to the opening motivation of this section? What is the answer that we found?}
We found that greater phonetic distortion in coded language was associated with higher rating prediction error, but this relationship varied across coded language categories and remained modest overall. 
The MSE between the GPT-5-mini predicted rating and the user-assigned rating are shown in the table \ref{tab:mse_by_class}.
%[\changye{not sure how to refer to this dataset - the full dataset? This dataset is bigger than the dictionary we used in the last few paragraphs, which explains the differences in CER below}] 
%reached 0.31, 0.43, 0.51, 0.56, 0.86 for Ambiguous Homophone, Non-Lexical Homophone, Phonetic Substitution, Emoji Substitution, and Cross-Lingual Phonetic Encoding, respectively.
%0.31, 0.86, 0.56, 0.43, 0.51 for Ambiguous Homophone, Cross-Lingual Phonetic Encoding, Emoji Substitution, Non-Lexical Homophone, and Phonetic Substitution, respectively. 
%The average Pinyin CER for each class yielded 0.49, 1.23, 0.58, 0.30, and 0.61, and the average IPA CER for each class yielded 0.57, 2.46, 0.63, 0.37, and 0.68, respectively. 
The Spearman's $\rho$ between MSE and average CER reached 0.80 for both Pinyin and IPA, suggesting that more character errors were associated with more variance between predicted ratings and user-assigned ratings. Yet, the correlations did not reach conventional levels of statistical significance (p-value = 0.104).
%neither correlation was statistically significant 
%\kenneth{What does this significance mean? Compared against what?} [\changye{the statistical strength of rho}]

The Cross-Lingual Phonetic Encoding class achieved the highest MSE and CER for both Pinyin and IPA, which may be due to the lack of cross-lingual context and the limited data size. %Interestingly, the Ambiguous Homophone and Non-Lexical Homophone classes reached a divergent pattern: one exhibited higher MSE but lower CER, whereas the other showed lower MSE but higher CER for both Pinyin and IPA. This suggests a dissociation between phonological similarity and semantic decoding across coded language categories. 
Compared to Ambiguous Homophones, Non-Lexical Homophones achieved lower CER under both Pinyin and IPA, but obtained higher MSE in rating prediction. This suggested that, despite higher pronunciation similarity, the loss of lexicalized meaning in Non-Lexical Homophones impairs downstream pragmatic interpretation more.
%Cross-lingual homophones were especially prone to surface plausibility but semantic mismatch,  producing rare forms, creative spellings, and code-mixed tokens. While some coded spans were phonetically distant from their canonical targets, the surrounding context (\eg, topic, sentiment indicators, and known internet slang patterns) may help decode the intended meaning, leading to a closer predicted rating than the user-generated rating and, subsequently, a lower MSE.
%\paragraph{Abbreviations and cross-lingual encoding distort pronunciation the most.}
%Figure~\ref{fig:cer} shows error type distributions across categories. 
%Ambiguous homophones and non-lexical homophones exhibited relatively low CER, while phonetic substitution and transliteration showed substantially higher CER. 
%Transliteration had the highest CER in both pinyin and IPA.

%Deletion errors were most frequent in the phonetic substitution category. This was largely caused by orthographic abbreviations, where multi-syllabic words were reduced to initials. For example, \texttt{rmb} abbreviated \texttt{ren2 min2 bi4}, but the initials lacked sufficient phonological information and often produced unknown tokens during IPA conversion. We also observed cross-lingual abbreviation cases such as \texttt{ww}, which originated from Japanese \textit{warai} and was used to mean \texttt{haha}.

%Substitution errors were the second most common error type across categories. These substitutions often replaced target sounds with phonetically similar but intentionally incorrect variants, reflecting deliberate phonetic interference rather than noise.




%\kenneth{-----------------KENNETH IS WORKING HERE; ORIGINAL draft below----------------}

%We annotate the pinyin\footnote{\url{https://github.com/mozillazg/python-pinyin}} and International Phonetic Alphabet (IPA)\footnote{\url{https://github.com/stefantaubert/pinyin-to-ipa}} for each pair of strings in the golden standard data, excluding the cipher and orthographic class [\changye{this refers to the coded\_dictionary\_w\_phonetics.csv file}]. The tones in pinyin are annotated from 1 to 4, and mapped to IPA (1 to \tone{55}, 2 to \tone{35}, 3 to \tone{313}, and 4 to \tone{51}), respectively. We adapt the character error rate (CER) from automatic speech recognition evaluation pipeline to quantify the structure deviations between the references (the decoded strings) and hypotheses (the coded strings) tokens. CER is derived from Levenshtein distance by normalizing the sum of substitutions, deletions, and insertions over the total number of characters given a pair of reference and hypothesis. In other words, we adapt CER to represent the \textit{proportion} of structural deviations for a pair of coded language strings, serving as a proxy for the degree of phonetic overlap. In this study, we calculate the CER for each pair on annotated pinyin and IPA separately for all coded language categories.






==> latex/sections/6-discussion.tex <==
% discuss the adaptation, representation, personalization and time-sensitivity in discussion 
% Effectiveness
% unique code
% common usage 
%interoretation boundary 
%\paragraph{Adaptation of Coded Language Over Time.}
\paragraph{Expressiveness vs. Interpretability in Coded Language.}
Our data shows a highly skewed distribution in coded language usage: 
%[\changye{this applies to our dataset only; does not apply to \textit{all} coded languages}] 
among 184 unique coded spans, 111 appear only once, while a small number of forms are used repeatedly. 
The most frequent span, ``\begin{CJK}{UTF8}{gbsn}滴\end{CJK}''(di1, drip), appears 102 times and serves as a phonetic substitution for ``\begin{CJK}{UTF8}{gbsn}的\end{CJK}''(de, of), often used to convey a playful, cute tone. 
This pattern suggests that while the majority of coded expressions are context-specific, a small subset becomes widely shared and stabilized through repeated use. 
This observation aligns with prior work showing that popular code words rely on unconventional character combinations and simple, memorable, affective, or sarcastic expressions~\cite{zhang2014appropriate}.
%Prior work has similarly observed that popular code words tend to have unconventional character combinations, affective or sarcastic expressions that are simple, memorable, and easily reusable by a broad audience~\cite{zhang2014appropriate}.
At the other extreme, some unique spans in our dataset were difficult even for human annotators to interpret. 
For example ``\includegraphics[height=1.2em]{latex/figures/elephant.png}\begin{CJK}{UTF8}{gbsn}人\end{CJK}\includegraphics[height=1.2em]{latex/figures/shen.png}\begin{CJK}{UTF8}{gbsn}一\end{CJK}\includegraphics[height=1.2em]{latex/figures/sheep.jpeg}\includegraphics[height=1.2em]{latex/figures/de.png}\begin{CJK}{UTF8}{gbsn}姜\end{CJK}'' used emojis to replace homophone words. 
The review reads as (xiang4 ren2 shen1 yi\textbf{1} yang\textbf{2} de\textbf{2} jiang1, elephant human apply one sheep get ginger), which actually means (xiang4 ren2 shen1 yi\textbf{2} yang\textbf{4} de jiang1, the ginger was like ginseng).

There is a trade-off between expressiveness and interpretability in coded language. 
Codes that are easy to recognize, humorous, or representative are more likely to be widely adopted and circulate as shared memes, but their obfuscatory or boundary-setting function weakens as they spread. 
In contrast, niche or opaque codes preserve stronger hiding effects but require greater interpretive effort and shared background knowledge. 
Prior work shows that human-created code words are perceived as funnier than machine-generated ones and are therefore more likely to be adapted over time~\cite{zhang2015context}. 
Similarly, \citet{wan2025hashtag} shows that boundary-making strategies based on linguistic tricks lose effectiveness as audiences diversify, forcing users to continually invent new, more creative, and less transparent codes. 
%Together, these findings show that simple codes spread easily but lose exclusivity, whereas rarer codes remain personalized, context-dependent, and harder to interpret.





%indicating a trade-off between expressiveness and interpretability. 
%Codes that are easy to recognize, humorous, or representative are more likely to be adopted by a wider community and evolve into shared memes; however, as their usage becomes widespread, their original obfuscatory or boundary-setting function diminishes. In contrast, more niche or opaque codes retain stronger hiding effects but require greater interpretive effort and shared background knowledge. Consistent with prior findings that human-created code words are perceived as funnier than machine-generated ones, such codes are also more likely to be reused and adapted over time \cite{zhang2015context}. \citet{wan2025hashtag} also shows that boundary-making strategies using language tricks tend to lose effectiveness as audiences diversify, prompting users to continually invent new, more creative, and less transparent codes. 
%Together, these observations highlight the evolving nature of coded language: Simple codes are more easily reused by a broad audience, whereas rarer coded expressions tend to remain highly personalized, context-dependent, and harder to interpret.

\paragraph{Multilingualism of Coded Language.} 
Our analysis further shows that coded language often operates across languages and writing systems, creating barriers to interpretation for both native speakers and language models.
Some coded expressions exploited cross-script visual similarity rather than phonetic or semantic equivalence, such as using Kanji or Chinese characters whose shapes resemble Latin letters (\eg, ``\begin{CJK}{UTF8}{gbsn}爪丫\end{CJK}'' encoding ``MY'').
%In some instances, coded expressions relied on visual similarity across scripts, such as the use of Kangji radicals or Chinese characters whose shapes resemble Latin letters (\eg, ``\begin{CJK}{UTF8}{gbsn}爪丫\end{CJK}'' encoding ``MY''), which applied cross-script visual resemblance rather than phonetic or semantic equivalence.  
More broadly, Chinese comprises a family of languages and dialects with varying alignments between written and spoken forms.
For example, written Cantonese closely reflects spoken Cantonese and differs substantially from Mandarin in syntax and lexicon, introducing additional variation in coded expressions.
%More broadly, Chinese itself encompasses a diverse family of languages and dialects, with written and spoken forms exhibiting varying degrees of alignment with alphabetic languages. 
%For example, Cantonese writing is closely tied to spoken Cantonese pronunciation and differs substantially from Mandarin in both syntax and lexicon, introducing additional layers of variation in coded expression. 
%Chinese online communication is also shaped by sustained contact with neighboring languages such as Japanese and Korean, leading to the use of transliterations to encode foreign expressions. 
Chinese online communication also draws on sustained contact with neighboring languages such as Japanese and Korean, leading to the use of transliteration-based codes.
For example, ``\begin{CJK}{UTF8}{gbsn}卡哇伊\end{CJK}'' (ka3 wa1 yi1, card wow they) means \begin{CJK}{UTF8}{min}かわいい\end{CJK} (Kawaii, cute) from Japanese. 
These multilingual and cross-script practices highlight that understanding coded language often requires shared community knowledge spanning multiple linguistic systems, further complicating both human annotation and automated interpretation.

==> latex/sections/7-conclusion.tex <==
Coded language is a common communicative strategy in which intended meaning diverges from surface form and requires decoding to be understood. We presented \dataset, a dataset of 7,744 Chinese Google Maps reviews with span-level annotations and a seven-class taxonomy capturing phonetic, orthographic, and cross-lingual encoding strategies. We evaluated language models on coded language detection, classification, and review rating prediction. Our results showed that even strong models frequently fail to detect coded language, and phonetic distortions contribute to downstream prediction errors. These findings highlight coded language as a persistent challenge for real-world NLP systems and motivate further work.

==> latex/tables/additional_classification.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lcccc}
\toprule
\textbf{Coded Language Class} & \textbf{P} $\uparrow$ & \textbf{R} $\uparrow$ & \textbf{F1} $\uparrow$  \\
\midrule
Ambiguous Homophone        & 0.66 & 0.61 & 0.63  \\
Non-Lexical Homophone      & 0.65 & 0.54 & 0.59  \\
Phonetic Substitution      & 0.50 & 0.95 & 0.65  \\
Emoji Substitution         & 0.75 & 0.25 & 0.38 \\
Cipher                     & 0.86 & 0.81 & 0.84 \\
Orthographic Substitution  & 0.30 & 0.91 & 0.45  \\
Cross-Lingual Phonetic Encoding & 0.05 & 1.00 & 0.10  \\

\bottomrule
\end{tabular}
\caption{Per-class coded language classification performance for \texttt{GPT-5-mini}.}
\label{tab:gpt_classification}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Coded Language Class} & \textbf{P} $\uparrow$ & \textbf{R} $\uparrow$ & \textbf{F1} $\uparrow$  \\
\midrule
Ambiguous Homophone & 0.57 & 0.61 & 0.59 \\
Non-Lexical Homophone & 0.68 & 0.73 & 0.70 \\
Phonetic Substitution & 0.51 & 0.97 & 0.67\\
Emoji Substitution & 0.77 & 0.83 & 0.80  \\
Cipher & 0.78 & 0.85 & 0.81 \\
Orthographic Substitution & 0.46 & 0.97 & 0.63 \\
Cross-Lingual Phonetic Encoding & 0.04 & 1.00 & 0.08 \\
\bottomrule
\end{tabular}
\caption{Per-class coded language classification performance for \texttt{Gemini-2.5-Flash}.}
\label{tab:gemini_classification}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Coded Language Class} & \textbf{P} $\uparrow$ & \textbf{R} $\uparrow$ & \textbf{F1} $\uparrow$ \\
\midrule
Ambiguous Homophone & 0.45 & 0.23 & 0.30 \\
Non-Lexical Homophone & 0.38 & 0.30 & 0.34 \\
Phonetic Substitution & 0.48 & 0.16 & 0.24 \\
Emoji Substitution & 0.10 & 0.08 & 0.09 \\
Cipher & 0.45 & 0.12 & 0.19 \\
Orthographic Substitution & 0.17 & 0.65 & 0.27 \\
Cross-Lingual Phonetic Encoding & 0.09 & 0.57 & 0.16 \\
\bottomrule
\end{tabular}
\caption{Per-class coded language classification performance for \texttt{Qwen2.5-7B-Instruct}.}
\label{tab:qwen_classification}
\end{table}


==> sections/1-Introduction.tex <==



\begin{comment}
 
\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{latex/figures/NE_example.pdf}
    \caption{Example of creative coded language in a Google Maps restaurant review. Left: the original user review in Chinese, as posted on Google Maps. Middle: the machine-generated English translation from Google Translate. Right: the hidden meaning decoded through phonetic substitutions.}
    \label{fig:NE}
\end{figure*}
   
\end{comment}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{latex/figures/CodedLang_Concept.png}
    \caption{Example of creative coded language in a Google Maps restaurant review. Top: the original user review in Chinese, as posted on Google Maps. Left: the machine-generated English translation produced by Google Translate. Right: the inferred underlying meaning obtained by decoding phonetic substitutions.}
\label{fig:NE}
\end{figure}

Coded language is an important way people communicate with each other~\cite{ji2018creative}.
Instead of expressing meaning directly, writers intentionally encode their intent so that the surface text differs from the intended meaning and must be decoded by an informed reader. 
Such practices are common in everyday communication, yet they remain understudied in natural language processing (NLP), where models typically assume that meaning is conveyed transparently in literal text.

Online review platforms provide a clear real-world context in which coded language emerges.
While reviews influence consumer decisions and public reputation, writing negative reviews can expose users to social pressure, retaliation, or reduced visibility. 
Among Chinese-speaking users on Google Maps, we observed a recurring strategy: embedding negative evaluations inside seemingly positive or neutral reviews using coded language. 
These reviews rely on homophones, phonetic substitutions, transliteration, emoji, and cross-lingual cues that obscure meaning from casual readers, machine translation systems, and moderation tools, while remaining interpretable to in-group audiences.
For example, a review stating ``\textbf{Newspaper eat}'' appears nonsensical in English but encodes a negative message through a phonetic substitution of the Chinese phrase ``\begin{CJK}{UTF8}{gbsn}不好吃\end{CJK}'' (bu4 hao3 chi1, meaning \textbf{not tasty}). 
When spoken quickly, ``bu4 hao3 chi1'' can sound like ``bao4 chi1'' (\begin{CJK}{UTF8}{gbsn}报吃\end{CJK}), which literally translates to ``Newspaper Eat'' in English, where ``bao4'' means newspaper and ``chi1'' means eat.
Figure~\ref{fig:NE} shows another representative example, where machine translation systems fail to recover the intended meaning. %and often produce misleadingly positive outputs. 
These examples illustrate how coded language creates a systematic gap between surface form and communicative intent that current NLP systems struggle to bridge.

To study this phenomenon, we curated \textbf{\dataset}, a dataset of 7,744 real-world Chinese Google Maps reviews, including \textbf{900 reviews containing coded language with span-level annotations} (Section~\ref{sec:data}). 
%Based on these annotations, 
We also developed a seven-class taxonomy that captures common encoding strategies, including homophonic, phonetic, and cross-lingual substitutions (Section~\ref{sec:taxonomy}). 
Using \dataset, we evaluated modern language models on three NLP tasks (Section~\ref{sec:evaluation})
%coded language detection, classification, 
%and review rating prediction, 
and further analyzed the phonetic properties of coded expressions (Section~\ref{sec:analysis}).
This work treats coded language as a systematic and understudied form of real-world communication and provides a grounded dataset and taxonomy for examining how NLP systems handle intentionally encoded meaning in practice.

%-------------------------------- dead kitten --------------------

\begin{comment}
    

%\kenneth{---------------KENNETH IS WORKING HERE-------------------}

Online review platforms play a crucial role in shaping consumer decisions by allowing users to share their experiences. Authentic reviews help build trust within these communities, benefiting both consumers and business owners. However, sharing negative experiences introduces complex dynamics, especially when users face risks of social burden, retaliation, or reduced visibility due to platform algorithms. 
Among Chinese-speaking users, a creative strategy has emerged: embedding negative content within seemingly positive or neutral Google Maps reviews using coded language. These reviews rely on linguistic variations, homophones, transliteration, and cultural references that bypass detection by non-Chinese readers, machine translation, and moderation systems. For example, a review stating “Newspaper eat” appears nonsensical in English but encodes negative message through a phonetic substitution of the Chinese phrase ``\begin{CJK}{UTF8}{gbsn}不好吃\end{CJK}'' (bù hǎo chī, meaning not tasty). When spoken quickly, “bù hǎo chī” can sound like “bào chī”(\begin{CJK}{UTF8}{gbsn}报吃\end{CJK}), which literally translates to “Newspaper Eat” in English, where “bào” means newspaper and “chī” means eat. 

Figure~\ref{fig:NE} also shows another example, highlighting the complexity and creativity behind such coded reviews. On the left is the original Chinese-language review as posted on Google Maps, including exaggerated praise and heart emojis. The middle shows the machine-generated English translation from Google Translate. On the right is a manually decoded version by myself [\changye{I wouldn't recommend to use \textit{myself} here. How about \textit{authors}?}], translated based on phonetic substitutions and contextual slang, revealing the hidden negative sentiment. Notably, machine translation fails to capture the intended meaning. For instance, phrases like ``terrible meals'' are translated as ``delicious meals,'' ``lie'' becomes ``good,'' ``doesn’t exist'' appears as ``charming,'' and ``don’t come'' is misrepresented as ``tonic.'' These coded expressions convey criticism only interpretable by Chinese readers familiar with the trick. This practice shows the challenges of multilingual communication online. [\changye{should we mention the contributions here?}]


\end{comment}
